GRAPHMOE: Amplifying Cognitive Depth of Mixture-of-Experts Network via Introducing Self-Rethinking Mechanism

Traditional Mixture-of-Experts (MoE) networks benefit from utilizing multiple smaller expert models as opposed to a single large network. However, these experts typically operate independently, leaving a question open about whether interconnecting these models could enhance the performance of MoE networks. In response, we introduce GRAPHMOE, a novel method aimed at augmenting the cognitive depth of language models via a self-rethinking mechanism constructed on Pseudo GraphMoE networks. GRAPHMOE employs a recurrent routing strategy to simulate iterative thinking steps, thereby facilitating the flow of information among expert nodes. We implement the GRAPHMOE architecture using Low-Rank Adaptation techniques (LoRA) and conduct extensive experiments on various benchmark datasets. The experimental results reveal that GRAPHMOE outperforms other LoRA based models, achieving state-of-the-art (SOTA) performance. Additionally, this study explores a novel recurrent routing strategy that may inspire further advancements in enhancing the reasoning capabilities of language models.

==> tables/overhead_analysis.tex <==
\begin{table}[htbp]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccc|c}
    \toprule
    \textbf{Task} & \textbf{Scaling Factor $\overline{d}/{d}$} & \textbf{Param/\%}  & \textbf{Acc./\%} & \textbf{Acc. Diff/\%} \\
    \midrule
    \multirow{5}{*}{ARC-E} 
    & 0.01 & 3.3 & 88.3 & 0.0 \\
    & 0.02 & 3.5 & 88.6 & 0.3 \\
    & 0.05 & 4.4 & 88.4 & 0.1 \\
    & 0.1  & 5.9 & 89.2 & \textbf{0.9} \\
    & 0.2  & 9.2 & 89.2 & \textbf{0.9} \\
    \midrule
    \multirow{5}{*}{ARC-C} 
    & 0.01 & 3.3 & 80.5 & 0.0 \\
    & 0.02 & 3.5 & 80.6 & 0.1 \\
    & 0.05 & 4.4 & 80.1 & -0.4 \\
    & 0.1  & 5.9 & 80.9 & \textbf{0.4} \\
    & 0.2  & 9.2 & 79.8 & -0.7 \\
    \bottomrule
\end{tabular}
}
\caption{Impact of GRU Hidden Size Scaling Factor $\overline{d}/{d}$ on Parameter Efficiency and Accuracy Across Tasks.}
\label{tab:overhead_analysis_zzf}
\end{table}
